On The Role of Alias and Band-Shift for Sentinel-2 Super-Resolution

In this work, we study the problem of single-image super-resolution (SISR) of Sentinel-2 imagery. We show that thanks to its unique sensor specification, namely the inter-band shift and alias, that deep-learning methods are able to recover fine details. By training a model using a simple $L_1$ loss, results are free of hallucinated details. For this study, we build a dataset of pairs of images Sentinel-2/PlanetScope to train and evaluate our super-resolution (SR) model.

==> img/many-results/airport-Gr_g_b.tex <==
33.31


==> img/many-results/airport-Grgb.tex <==
33.58


==> img/many-results/airport-Grgb_gan.tex <==
31.97


==> img/many-results/airport-Grgb_gan_pretrained.tex <==
31.94


==> img/many-results/airport-bicubic.tex <==
32.10


==> img/many-results/parking-Gr_g_b.tex <==
36.34


==> img/many-results/parking-Grgb.tex <==
38.38


==> img/many-results/parking-Grgb_gan.tex <==
32.91


==> img/many-results/parking-Grgb_gan_pretrained.tex <==
34.43


==> img/many-results/parking-bicubic.tex <==
32.78


==> img/many-results/suburbs-Gr_g_b.tex <==
35.43


==> img/many-results/suburbs-Grgb.tex <==
37.90


==> img/many-results/suburbs-Grgb_gan.tex <==
35.11


==> img/many-results/suburbs-Grgb_gan_pretrained.tex <==
35.62


==> img/many-results/suburbs-bicubic.tex <==
34.01


==> img/many-results/tanks-Gr_g_b.tex <==
25.87


==> img/many-results/tanks-Grgb.tex <==
26.79


==> img/many-results/tanks-Grgb_gan.tex <==
24.64


==> img/many-results/tanks-Grgb_gan_pretrained.tex <==
24.98


==> img/many-results/tanks-bicubic.tex <==
25.19


==> img/many-results/tanks2-Gr_g_b.tex <==
30.49


==> img/many-results/tanks2-Grgb.tex <==
32.13


==> img/many-results/tanks2-Grgb_gan.tex <==
27.49


==> img/many-results/tanks2-Grgb_gan_pretrained.tex <==
28.77


==> img/many-results/tanks2-bicubic.tex <==
27.75


==> img/many-results/worksite-Grgb_gan.tex <==
30.56

